HAPM -- Hardware Aware Pruning Method for CNN hardware accelerators in resource constrained devices

During the last years, algorithms known as Convolutional Neural Networks (CNNs) had become increasingly popular, expanding its application range to several areas. In particular, the image processing field has experienced a remarkable advance thanks to this algorithms. In IoT, a wide research field aims to develop hardware capable of execute them at the lowest possible energy cost, but keeping acceptable image inference time. One can get around this apparently conflicting objectives by applying design and training techniques. The present work proposes a generic hardware architecture ready to be implemented on FPGA devices, supporting a wide range of configurations which allows the system to run different neural network architectures, dynamically exploiting the sparsity caused by pruning techniques in the mathematical operations present in this kind of algorithms. The inference speed of the design is evaluated over different resource constrained FPGA devices. Finally, the standard pruning algorithm is compared against a custom pruning technique specifically designed to exploit the scheduling properties of this hardware accelerator. We demonstrate that our hardware-aware pruning algorithm achieves a remarkable improvement of a 45 % in inference time compared to a network pruned using the standard algorithm.

==> 01-introduction_min.tex <==
\section{Introducción}

Este trabajo plantea como hipótesis que una implementación dedicada de una arquitectura de hardware específicamente diseñada para ejecutar redes neuronales convolucionales es capaz de lograr una performance comparable a la de un hardware clásico (CPU o GPU), con un consumo de energía menor y por lo tanto, una relación costo/beneficio mayor. Por lo tanto, se investigó el estado del arte de las implementaciones sobre hardware existentes de las operaciones básicas de una red neuronal convolucional y se compararon para seleccionar las que mejor se adecúen a las necesidades del proyecto. Utilizando la investigación realizada, se implementaron los módulos básicos que permitan resolver las operaciones de una red neuronal convolucional y con ellos se conformó una arquitectura de hardware genérica configurable, capaz de ejecutar redes neuronales con distintos parámetros. Finalmente, se validó el comportamiento del diseño realizado ejecutando múltiples versiones de una red neuronal previamente entrenada con distintas técnicas, con el objetivo de comparar los resultados y extraer conclusiones sobre la conveniencia de aplicar ciertos algoritmos de entrenamiento y su impacto en la velocidad de predicción de la red neuronal sobre el hardware implementado.

%Se inicia este trabajo con una sección donde se presentan trabajos previos y conceptos relacionados con este desarrollo. Dentro del mismo se realiza una introducción a las redes neuronales convolucionales y se referencian otros trabajos de investigación sobre implementaciones de este tipo de algoritmos sobre FPGA. Luego se prosigue con una sección que explica en detalle el funcionamiento interno del diseño de hardware realizado. La siguiente sección explica la selección de una red neuronal convolucional específica, utilizada para validar el funcionamiento del diseño, junto con las distintas versiones entrenadas de la misma. A continuación se presentan las mediciones realizadas sobre el hardware diseñado utilizando las versiones entrenadas en la sección anterior. Finalmente, se presentan las conclusiones extraídas.

==> 02-marcoteorico_min.tex <==
\spanish{\section{Trabajo previos}}
\english{\section{Previous work}}

\spanish{\subsection{Redes neuronales convolucionales}}
\english{\subsection{Convolutional Neural Networks}}

\spanish{Una red neuronal suele definirse como un aproximador universal de funciones. El modelo básico conocido como \textit{perceptrón multicapa} consta de una sucesión de $k$ capas de \textit{neuronas} interconectadas de forma secuencial, donde la salida de una determinada neurona $j$ viene dada por la suma ponderada de todas las salidas de las neuronas de la capa anterior, más un valor de bias $b_{j}$.} %Los valores $w_{ij}$ que ponderan las entradas de la neurona y los valores de bias $b_{j}$ se conocen como los \textit{pesos} o \textit{coeficientes} de una red neuronal. Este tipo de capas de neuronas se conocen como \textit{fully connected} (es decir, completamente conectadas), ya que la salida de una determinada neurona de la capa $k$ se calcula utilizando todas las salidas de las neuronas de la capa anterior. 
\english{A neural network is usually defined as an universal function approximator. The basic model known as the \textit{multilayer perceptron} consists of a succession of $k$ layers of \textit{neurons} interconnected in a sequential manner, where the output of a given neuron $j$ is given by the weighted sum of all the outputs of the neurons of the previous layer, plus a bias value $b_{j}$.}
    
%\subsection{Redes neuronales convolucionales}
%\label{section:cnn}

% Que es una red neuronal convolucional
\spanish{Una capa convolucional es una extensión de los conceptos anteriores, donde la salida de cada neurona viene dada sólo por la suma ponderada de un determinado grupo de las salidas de la capa anterior. Conceptualmente, las salidas de una determinada capa convolucional pueden interpretarse como el resultado de desplazar $N_{of}$ filtros de dimensiones $N_{kx}\times N_{ky}\times N_{if}$ por las salidas de la capa anterior, y en cada desplazamiento del filtro se realiza la suma ponderada de las salidas de la capa anterior por los coeficientes del filtro.}% (el algoritmo \ref{al:conv} presenta en pseudocódigo cómo se calcula la salida de una capa de este tipo). %Para este caso, los coeficientes de los $N_{of}$ filtros de una capa convolucional se conocen como los \textit{pesos} de esa capa.
\english{A convolutional layer is an extension of the previous concepts, where the output of each neuron is given only by the weighted sum of a certain sub-set of the outputs of the previous layer. \todo{explicar mejor los valores}The outputs of a certain convolutional layer can be interpreted as the result of shifting $N_ {of}$ filters of dimensions $N_ {kx} \times N_{ky} \times N_{if} $ over the outputs of the previous layer, and at each filter displacement step the weighted sum of the outputs of the previous layer is performed, using the filter coefficients as weights.}

%    \begin{itemize}
%        \item $N_{if}$: cantidad de canales de la matriz de entrada a la capa
%        \item $N_{ix}$: ancho de la matriz de entrada a la capa
%        \item $N_{iy}$: alto de la matriz de entrada a la capa
%        \item $N_{kx}$: ancho de cada filtro de la capa
%        \item $N_{ky}$: alto de cada filtro de la capa
%        \item $N_{of}$: cantidad de canales de la matriz de salida de la capa (es igual a la cantidad de grupos de filtros de la capa)
%        \item $N_{ox}$: ancho de la matriz de salida de la capa
%        \item $N_{oy}$: alto de la matriz de salida de la capa
%        \item $k_{[...]}^{...}$: matriz de coeficientes de los grupos de filtros de la capa
%        \item $b^{...}$: bias de los grupos de filtros de la capa a calcular
%        \item $stride_{...}$: también conocido como \textit{paso}, indica el desplazamiento de los filtros tanto en el eje x como en el eje y
%        \item $padding_{...}$: representa la cantidad de filas (arriba y abajo) o columnas (derecha e izquierda) de valores en cero que se agregan a la matriz de entrada de una capa convolucional, y que se utilizan para controlar el tamaño de la matriz de salida de la capa, como se puede ver en la ecuación \ref{eq:salida_conv} que describe cómo se calcula el tamaño en ancho y en alto de la matriz de salida de una capa convolucional, teniendo en cuenta el ancho y el alto de la matriz de entrada, el paso de los filtros, el ancho y alto de los filtros utilizados en la capa, y el \textit{padding}.
%    \end{itemize}

 %   \begin{algorithm*}
 %       \caption{Capa convolucional en pseudocódigo}\label{al:conv}
 %       \begin{algorithmic}[1]
 %           \State $o_{[..,..,..]} \leftarrow 0$\Comment{Inicialización de la matriz de salida en cero}
 %           \For{$f\gets0$ to $N_{of}-1$ by $1$}\Comment{Selector de grupo de filtro}
 %               \For{$i\gets0$ to $N_{ix}+2*padding_{x}-1$ by $stride_{x}$}\Comment{Eje x de entrada}
 %                   \For{$j\gets0$ to $N_{iy}+2*padding_{y}-1$ by $stride_{y}$} \Comment{Eje y de entrada}
 %                       \For{$k\gets0$ to $N_{if}-1$ by $1$}\Comment{Canales de entrada}
 %                           \For{$i_{k}\gets0$ to $N_{kx}-1$ by $1$}\Comment{Eje x del filtro seleccionado}
 %                               \For{$j_{k}\gets0$ to $N_{ky}-1$ by $1$}\Comment{Eje y del filtro seleccionado}
 %                                   \State $o_{[i,j,f]} \leftarrow o_{[i,j,f]} + i_{[i+i_{k},j+j_{k},k]} \cdot k_{[i_{k},j_{k},k]}^{f}$
 %                               \EndFor
 %                           \EndFor
 %                       \EndFor
 %                       \State $o_{[i,j,f]} \leftarrow o_{[i,j,f]} + b^{f}$
 %                   \EndFor
 %               \EndFor
 %           \EndFor
 %       \end{algorithmic}
 %   \end{algorithm*}
%
%    \begin{equation} \label{eq:salida_conv}
%        \begin{aligned}
%        N_{ox} = \frac{N_{ix}-N_{kx}+2*padding_{x}}{stride_{x}}+1 \\
%        N_{oy} = \frac{N_{iy}-N_{ky}+2*padding_{y}}{stride_{y}}+1
%        \end{aligned}
%    \end{equation}

% Se entiende por arquitectura de una red neuronal convolucional a la sucesión de capas convolucionales (y capas auxiliares) que se interconectan entre si para obtener un resultado a partir de una entrada determinada. 

\spanish{\subsection{Compresión de redes neuronales}}
\english{\subsection{Neural network compression}}
\label{section:marcoteorico_pruning}

\spanish{Una vez entrenados, estos algoritmos pueden sufrir algún tipo de optimización específica para el hardware sobre el cual se ejecutan. Una de las técnicas más utilizadas, es la de \textit{pruning} por valor absoluto \cite{DBLP:journals/corr/HanPTD15,DBLP:journals/corr/NarangDSE17,DBLP:journals/corr/SeeLM16}. La idea conceptual detrás de este algoritmo es que debido a la cantidad enorme de parámetros que suele tener una red neuronal, muchos de ellos son redundantes entre sí. Por lo tanto, un cierto número de parámetros pueden forzarse a cero, induciendo mayor \textit{sparsity} a la red neuronal. Esto resulta ventajoso en dos sentidos: se disminuye la cantidad de operaciones matemáticas que deben utilizarse para realizar una predicción, y en consecuencia se reducen los accesos a memoria debido a que hay menos coeficientes que leer.}
\english{Once trained, these algorithms can undergo different kinds of optimizations according to the hardware on which they will be executed. One of the most used techniques is the absolute value \textit{pruning} \cite{DBLP:journals/corr/HanPTD15,DBLP:journals/corr/NarangDSE17,DBLP:journals/corr/SeeLM16}. The intuitive idea behind this algorithm is that due to the enormous number of parameters that a neural network usually has, many of them are redundant. Therefore, a certain number of parameters could be forced to zero, inducing greater \textit{sparsity} to the neural network. This presents two advantages: it decreases the number of mathematical operations that must be executed to make a forward pass of the algorithm, and consequently reduces the needed memory accesses because there are fewer coefficients to read.}

\spanish{En este trabajo, se utilizó como \textit{baseline} la técnica propuesta por Zhu M. et. al. \cite{zhu2017prune} que consiste en forzar gradualmente coeficientes de cada capa a cero (hasta llegar a un cierto nivel de \textit{sparsity} deseado) mientras se reentrena para acomodar los parámetros restantes y así mantener la calidad de la predicción.}
\english{In this work, we used the technique proposed by Zhu M. et. al. \cite{zhu2017prune} as a baseline. This consists of gradually forcing coefficients of each layer to zero (until the amout of zero coefficients reaches a certain \textit{sparsity} threshold) while retraining to accommodate the remaining parameters and thus maintaining the quality of the prediction.}

\spanish{\subsection{Aceleradores de hardware}}
\english{\subsection{Hardware accelerators}}
\label{section:marcoteorico_aceleradores}

\spanish{Los aceleradores de hardware son desarrollos que se refieren al diseño de arquitecturas de hardware que permiten ejecutar una red neuronal en modo de inferencia (o predicción). Es decir, se entrena la red primero sobre una GPU o CPU, y luego se la utiliza sobre un hardware dedicado solamente para predecir. Este tipo de soluciones trabajan normalmente en conjunto con un microcontrolador o microprocesador que se encarga de: obtener los datos a analizar, enviarlos al hardware que la procesa de forma altamente eficiente, recibir el resultado del procesamiento y actuar en consecuencia. Este tipo de desarrollos presenta desafíos muy distintos a los desafíos encontrados durante el entrenamiento de la red neuronal ya que el enfoque está puesto en la forma más eficiente de ejecutar las operaciones internas de la red neuronal.}
\english{Hardware accelerators refer to the design of hardware architectures that allow a neural network to run in inference (or prediction) mode. That is, the network is trained first on a GPU or CPU, and then it is used on dedicated hardware only to predict. These kind of solutions normally work in conjunction with a microcontroller or microprocessor which is responsible for: obtaining the data to be analyzed, sending it to the hardware which is going to process it in a highly efficient way, receiving the processed result and acting accordingly. This kind of development presents challenges that are very different from the challenges encountered during neural network training since the main focus is to find the most efficient way of executing the internal operations needed for a forward pass (inference).}

\spanish{Existe un gran interés en el desarrollo de este tipo de arquitecturas, sobre todo para comparar la eficiencia y el consumo de redes neuronales implementadas sobre hardware contra implementaciones utilizando CPUs o GPUs, con el objetivo de implementar estos algoritmos en aplicaciones de bajo consumo \cite{DBLP:journals/corr/abs-1906-11879}. Otras investigaciones exploraron distintos tipos de arquitecturas para implementar este tipo de algoritmos sobre FPGAs \cite{DBLP:journals/corr/abs-1711-05860,Wielgosz_2019,Lozito}. Finalmente, existe también un amplio campo de investigación centrado exclusivamente en las formas de mejorar la eficiencia del cálculo de la convolución en hardware \cite{10.1145/3020078.3021727,aleks2018hardwareefficient,10.1145/3020078.3021736}, ya que según un análisis realizado por investigadores de la Universidad de Tsinghua (China), el 98 \% de las operaciones matemáticas que realizan las arquitecturas más utilizadas actualmente se dan en las capas convolucionales \cite{DBLP:journals/corr/abs-1712-08934}.}
\english{There is great interest in the development of this kind of architectures, especially to compare the efficiency and consumption of neural networks implemented on hardware against implementations using CPUs or GPUs, with the aim of implementing these algorithms in low-power applications \cite{DBLP:journals/corr/abs-1906-11879}. Other works explored different architectures to implement this kind of algorithms on FPGAs \cite{DBLP:journals/corr/abs-1711-05860,Wielgosz_2019,Lozito}. Finally, there is also a wide field of research focused exclusively on ways to improve the efficiency of the convolution output calculation in hardware \cite{10.1145/3020078.3021727,aleks2018hardwareefficient,10.1145/3020078.3021736}, since according to an analysis carried out by researchers from Tsinghua University (China), 98 \% of the mathematical operations performed by the nowadays most commonly used architectures are done in the convolutional layers \cite{DBLP:journals/corr/abs-1712-08934}.}

\spanish{A su vez, cuando se analiza este tipo de diseños, se suelen observar ciertas características como las analizadas en el trabajo de Ma et. al. \cite{10.1145/3020078.3021736}:}
\english{Furthermore, during the development of this kind of digital designs, certain characteristics are usually observed and taken into account as key aspects which need to be analyzed, such as those described in the work of Ma et. al. \cite{10.1145/3020078.3021736}:}

\spanish{
\begin{itemize}
	\item \textbf{Latencia(tiempo de procesamiento)}
	\item \textbf{Almacenamiento de sumas parciales}
	\item \textbf{Cantidad de accesos a los buffers internos:} lo cual determina 2 tipos de reutilizamiento de datos: reutilizacmiento espacial y temporal.
	\item \textbf{Cantidad de accesos a los buffers externos}
\end{itemize}}

\english{
	\begin{itemize}
		\item Latency (processing time)
		\item Storage of partial sums
		\item Number of accesses to internal buffers, which specifies 2 different types of data reuse: spatial reuse and temporal reuse.
		\item Number of accesses to external buffers
\end{itemize}}

\spanish{Por otro lado, los trabajos \cite{10.1007/978-3-030-05677-3_16,isscc_2016_chen_eyeriss} analizan la estructura de un elemento de procesamiento óptimo. Proponen que internamente estén conformados por un multiplicador y un sumador utilizado como acumulador. Estos elementos de procesamiento se interconectan de forma matricial para formar una estructura de tipo \textit{Systolic Array} \cite{1653825}, donde los coeficientes de un elemento de procesamiento son compartidos por otros elementos de procesamiento adyacentes, y lo mismo ocurre para los pixeles de entrada. A su vez, se propone que cada elemento de procesamiento tenga un mínimo control interno para poder seleccionar cuando acumular la suma interna y cuando enviar el resultado parcial a un elemento de procesamiento adyacente.}
\english{On the other hand, works like Yang et. al. \cite{10.1007/978-3-030-05677-3_16} and Chen et. al. \cite{isscc_2016_chen_eyeriss} analyze the structure of an optimal processing element. According to this works, this could be achieved by using a multiplier and an adder used as an accumulator. In order to maximize the internal data reuse, these works propose to interconnect this processing elements matrixically conforming a \textit{Systolic Array} \cite{1653825}, where the coefficients are shared across adjacent elements, and the same is true for the input pixels. Finally, it is proposed that each processing element should have a minimum internal control to be able to implement different kinds of operations.}

==> 03-arquitectura_min.tex <==
\spanish{\section{Arquitectura de hardware diseñada}}
\english{\section{Design of the hardware architecture}}

\spanish{Para el desarrollo realizado se utilizó una placa Zybo provista por el Departamento de Electrónica de la Facultad Regional Buenos Aires de la Universidad Tecnológica Nacional. La misma se encuentra basada en el chip Z-7010 de la familia Zynq de Xilinx, e integra dentro del mismo chip un \textit{hardcore processor} ARM Cortex-A9 \textit{dual core} capaz de trabajar con frecuencias de clock de hasta 866 MHz junto con una FPGA de la serie Artix-7 de Xilinx en tecnología de 28 nm. A los fines de este trabajo, la placa de desarrollo Zybo cuenta con 512 MB de memoria RAM DDR3 externa, mientras que internamente el chip cuenta con 240 KB de Block RAM y 80 \textit{DSP slices} \footnote{Para más información dirigirse a \url{https://reference.digilentinc.com/reference/programmable-logic/zybo/start}}.}
\english{In this work, a Zybo \footnote{For more information on the Zybo develpment board, please visit \url{https://reference.digilentinc.com/reference/programmable-logic/zybo/start}} and a Zedboard \footnote{For more information on the Zedboard develpment board, please visit \url{https://digilent.com/reference/programmable-logic/zedboard/start}} boards were used to carry out the development.}

\spanish{\subsection{Optimización de la operación de convolución}}
\english{\subsection{Optimization of the convolution operation}}
\label{section:conv_opt}

\begin{algorithm*}
	\scriptsize
	\caption{\spanish{Capa convolucional en pseudocódigo}\english{Pseudocode of a convolutional layer}}\label{al:conv}
	\begin{algorithmic}[1]
		\State $o_{[..,..,..]} \leftarrow 0$\Comment{\spanish{Inicialización de la matriz de salida en cero}\english{Initialization of the output matrix}}
		\For{$f\gets0$ to $N_{of}-1$ by $1$}\Comment{\spanish{Selector de grupo de filtro}\english{Filter group selector}}\label{lst:group_selector}
			\For{$i\gets0$ to $N_{ix}+2*padding_{x}-1$ by $stride_{x}$}\Comment{\spanish{Eje x de entrada}\english{Loop over the X axis of the input matrix}}
				\State $i_{o} \leftarrow i/stride_{x}$
				\For{$j\gets0$ to $N_{iy}+2*padding_{y}-1$ by $stride_{y}$} \Comment{\spanish{Eje y de entrada}\english{Loop over the Y axis of the input matrix}}\label{lst:y_axis}
					\State $j_{o} \leftarrow j/stride_{y}$
					\For{$k\gets0$ to $N_{if}-1$ by $1$}\Comment{\spanish{Canales de entrada}\english{Loop over the channels of the input matrix}}
						\For{$i_{k}\gets0$ to $N_{kx}-1$ by $1$}\Comment{\spanish{Eje x del filtro seleccionado}\english{Loop over the X axis of the selected filter}}\label{lst:x_kernel}
							\For{$j_{k}\gets0$ to $N_{ky}-1$ by $1$}\Comment{\spanish{Eje y del filtro seleccionado}\english{Loop over the Y axis of the selected filter}}\label{lst:y_kernel}
								\State $o_{[i_{o},j_{o},f]} \leftarrow o_{[i_{o},j_{o},f]} + i_{[i+i_{k},j+j_{k},k]} \cdot k_{[i_{k},j_{k},k,f]}$ \Comment{\spanish{Operación MACC}\english{MACC operation}}
							\EndFor
						\EndFor
					\EndFor
					\State $o_{[i_{o},j_{o},f]} \leftarrow o_{[i_{o},j_{o},f]} + b_{[f]}$ \Comment{\spanish{Suma del \textit{bias}}\english{\textit{Bias} sum}}
				\EndFor
			\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm*}

\spanish{El resultado de un capa convolucional puede calcularse utilizando una serie de ciclos anidados, tal como se presenta en el algoritmo \ref{al:conv}. Pero en una FPGA, estos ciclos se pueden paralelizar de distintas formas. En el trabajo de Yufei Ma et. al. \cite{10.1145/3020078.3021736} se analiza el impacto de 3 maneras de implementar estos ciclos:}
\english{The output of a convolutional layer can be calculated using a series of nested loops, as presented in algorithm \ref{al:conv}. But in a FPGA, these loops can be parallelized in different ways. In the work by Ma et. al. \cite{10.1145/3020078.3021736} the impact of 3 ways of implementing these cycles is analyzed, and this is how this strategies were used in this work:}

\spanish{
\begin{itemize}
	\item \textit{Loop unrolling}: En esta técnica se analiza qué ciclo del algoritmo es conveniente paralelizar con el fin de maximizar la cantidad de datos reutilizados y minimizar los accesos a memoria.
	\item \textit{Loop tiling}: En esta técnica se destaca que debido a la cantidad de datos de coeficientes y de salidas intermedias que tiene una red neuronal convolucional normalmente no es suficiente con la memoria interna del chip, y ciertos datos deben guardarse en DRAMs externas. Por lo tanto, con esta técnica se particionan los ciclos en bloques que sean lo suficientemente pequeños como para entrar en la memoria interna, pero lo suficientemente grandes como para minimizar la cantidad de intercambios de datos entre la memoria interna de la FPGA y la memoria DRAM externa.
	\item \textit{Loop interchange}: En este punto se analiza el orden en el cual se ejecutan los ciclos en el diseño de hardware. Esto condiciona el movimiento de datos interno entre elementos de procesamiento (multiplicadores y acumuladores). 
\end{itemize}}
\english{
\begin{itemize}
	\item \textit{Loop unrolling}: in this work, the loop at line \ref{lst:group_selector} was unrolled, and the design has the flexibility to unroll it fully or partially, depending on the amount of FPGA resources available. Loops at lines \label{lst:y_axis},\label{lst:x_kernel} and \label{lst:y_kernel} were also partially unrolled.
	\item \textit{Loop tiling}: in this work, the design can be configured to select which layers have their coefficients stored in the internal buffers of the FPGA (Block RAM) and which layers have their coefficients stored in the external RAM. In the latter case, the coefficients are first brought to the internal buffers before starting to execute the layer.
	%\item \textit{Loop interchange}: Here, the order in which the cycles are executed in the hardware design is analyzed. This conditions the internal data movement between processing elements (multipliers and accumulators). A suitable loop interchange strategy should be used to get the most out of the designed processing elements.
\end{itemize}}

\spanish{\subsubsection{Unidad de cómputo básica}}
\english{\subsubsection{Core processing element}}

\spanish{Recordando el algoritmo \ref{al:conv}, la operación básica que se realiza es de tipo MACC (multiplicar y acumular). Es por ello que utilizando como referencia los trabajos \cite{10.1007/978-3-030-05677-3_16} y \cite{isscc_2016_chen_eyeriss}, se decidió implementar un \textit{elemento de procesamiento} (de ahora en más, PE) como el que se puede ver en la figura \ref{fig:pe}, el cual consta de un multiplicador y un sumador que pueden utilizarse tanto para acumular la salida de si mismo con el valor multiplicado, como para acumular la suma parcial que viene de otro PE conectado en cascada. El mismo cuenta con las siguientes entradas:}
\english{As stated in algorithm \ref{al:conv}, the basic operation is a MACC operation (multiply and accumulate). This is why using as reference the works \cite{10.1007/978-3-030-05677-3_16} and \cite{isscc_2016_chen_eyeriss}, a \textit{processing element} (from now on, PE) as seen in figure \ref{fig:pe} was implemented. This PE consists of a multiplier and an adder that can be used both to accumulate the output of itself with the multiplied value, or to accumulate the partial sum that comes from another cascaded PE. %It has the following inputs and outputs:
}

%\spanish{\begin{itemize}
%	\item \textbf{Entrada de datos:} se utiliza para ingresar los datos de las imágenes de entrada (para la primera capa) o las salidas de la capa anterior.
%	\item \textbf{Entrada de coeficientes de filtros:} se utiliza para ingresar los coeficientes de los filtros de la capa que se está procesando.
%	\item \textbf{Entrada de sumas parciales:} esta entrada se utiliza para sumar el bias del filtro de la capa convolucional a la salida, o para sumar salidas de otros procesamientos anteriores.
%	\item \textbf{Salida de sumas parciales:} por este puerto se obtiene la salida de la capa convolucional, o una salida parcial que aún necesita ser procesada más adelante.
%\end{itemize}}
%\english{\begin{itemize}
%		\item \textbf{Data input:} it is used to input the pixel data of the input images (for the first layer) or the output data of the previous layer.
%		\item \textbf{Filter coefficients input:} is used to enter the coefficients of the filters for the layer that is being processed.
%		\item \textbf{Partial sum input:} this input is used to add the bias of the convolutional layer filter to the output, or to add previously processed outputs.
%		\item \textbf{Partial sum output:} through this port, the output of the convolutional layer or a partial output that still needs to be processed later is obtained.
%\end{itemize}}

\spanish{
\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{Basic_Process_Element_PE.pdf}
	\caption{Esquema simplificado de un PE}
	\label{fig:pe}
\end{figure}}

\english{\begin{figure}[H]
	\centering
	\includegraphics[width=0.3\textwidth]{Basic_Process_Element_PE_eng.pdf}
	\caption{Simplified block diagram of a PE used in this work}
	\label{fig:pe}
\end{figure}}

\spanish{Cada PE dentro del diseño de hardware se implementó utilizando uno de los DSP48E1 \footnote{\url{https://www.xilinx.com/support/documentation/user_guides/ug479_7Series_DSP48E1.pdf}} dedicados que se encuentran dentro de todas las FPGAs de la serie 7 de Xilinx.}
\english{Each PE within the hardware design was implemented using one of the dedicated DSP48E1 \footnote{\url{https://www.xilinx.com/support/documentation/user_guides/ug479_7Series_DSP48E1.pdf}} found within all Xilinx 7-series FPGAs.}

\spanish{\subsubsection{Matriz de unidades de cómputo}}
\english{\subsubsection{Computation units matrix}}

\spanish{Con el fin de reutilizar datos para resolver la operación de convolución, se plantea una estructura como la presentada en la figura \ref{fig:sysarray} compuesta por múltiples PEs conectados en cascada, conformando una matriz de PEs de tipo \textit{array sistólico}. De esta forma se logra reutilizar los datos de entrada en múltiples PEs: las flechas verdes indican la reutilización de los coeficientes del filtro que se convoluciona con la imagen, y las flechas azules indican la reutilización de los datos de la imagen (o de la entrada de la capa) a convolucionar. Esta reutilización disminuye la cantidad de accesos a memoria implementando la reutilización espacial de datos descripta en la sección \ref{section:marcoteorico_aceleradores}.}
\english{In order to reuse data while executing the convolution operation, a structure like the one presented in figure \ref{fig:sysarray} was proposed, composed of multiple cascaded PEs remembering a \textit{systolic array}. By connecting the PEs in this way, it is possible to reuse the input data in multiple PEs: the green arrows indicate the reuse of the filter coefficients that convolve with the image, and the blue arrows indicate the reuse of the image data (or the input layer). This reuse decreases the number of memory accesses by implementing the \textit{spatial reuse} of data described in section \ref{section:marcoteorico_aceleradores}.}

\spanish{\begin{figure}
	\centering
	\includegraphics[width=0.2\textwidth]{SystolicArray.pdf}
	%\centering{
	%	\def\svgwidth{0.3\textwidth}
	%	\input{SystolicArray.pdf}
	%}
	\caption{Esquema básico de la matriz de PEs}
	\label{fig:sysarray}
\end{figure}}

\english{\begin{figure}[H]
	\centering
	\includegraphics[width=0.2\textwidth]{SystolicArray_eng.pdf}
	%\centering{
	%	\def\svgwidth{0.3\textwidth}
	%	\input{SystolicArray.pdf}
	%}
	\caption{Basic block diagram of an arrange of PEs, used to maximize the reutilization of coefficients and input data in a convolution operation}
	\label{fig:sysarray}
\end{figure}}

\spanish{\subsubsection{Bloque de matrices}}
\english{\subsubsection{Matrix block}}
\label{section:bloque_de_matrices}

\spanish{Se diseña este módulo que se encarga de instanciar $n$ matrices en paralelo como se puede ver en la figura \ref{fig:computation_block}. Para poder seleccionar el grado de paralelismo deseado y la cantidad de recursos utilizados por este módulo, se lo diseña con \textit{generics} que permiten sintetizarlo seleccionando la cantidad de matrices que se deben instanciar en paralelo y la profundidad de cada buffer FIFO. Expone los siguientes buses:}
\english{This module is designed to instantiate $n$ matrixes (like the ones presented in figure \ref{fig:sysarray}) in parallel as it is presented in figure \ref{fig:computation_block}. This is the module which actually executes the complete convolution operation, and by selecting the amount of $n$ matrixes it allows to control the desired parallelism level and the amount of resources used. Each matrix has a FIFO buffer in each of its inputs and output, in order to uncouple the processing of this module from the one that feeds it the data.}

%\spanish{\begin{itemize}
%	\item \textbf{Bus de datos de 32 bits:} todos los buffers FIFO de entrada de datos se encuentran conectados en paralelo a este bus, para que puedan ser cargados todos a la vez en el mismo ciclo de clock.
%	\item \textbf{Bus de coeficientes de 24 bits:} todos los buffers de coeficientes de filtros se encuentran conectados en paralelo a este bus, para que puedan ser cargados todos a la vez en el mismo ciclo de clock, en caso de que todos necesiten el mismo dato.
%	\item \textbf{Bus de entradas de sumas parciales de $16\cdot n$ bits:} se utiliza un bus con el tamaño suficiente para poder cargar en una sola escritura (un solo ciclo de clock), todos los buffers FIFO de entradas de sumas parciales.
%	\item \textbf{Bus de salidas de sumas parciales de $16\cdot n$ bits:} se utiliza un bus con el ancho suficiente para poder leer de una sola vez (un solo ciclo de clock), todos los buffers FIFO de salidas de sumas parciales.
%	\item Múltiples buses de control y estado: estos buses se utilizan para, entre otras cosas, monitorear desde el controlador los estados de los buffers de cada unidad de cómputo (para evitar lecturas de buffers vacíos o escrituras de buffers llenos), parametrizar cada unidad, enviar la señal de inicio a cada matriz, etc.
%\end{itemize}}
%\english{\begin{itemize}
%		\item \textbf{32 bit data bus:} all data FIFO buffers are connected in parallel to this bus, in order to load them all together in the same clock cycle.
%		\item \textbf{24 bit coefficient bus:} all filter coefficient buffers are connected in parallel to this bus, so that they can all be loaded in the same clock cycle, in case they all need the same data.
%		\item \textbf{16*n bits input partial sum bus:} a bus of sufficient size is used to be able to load in a single write (a single clock cycle), all the FIFO buffers of partial sum inputs.
%		\item \textbf{16*n bits output partial sum bus:} a bus with sufficient width is used to be able to read in a single time (a single clock cycle), all the FIFO buffers of partial sums outputs.
%		\item \textbf{Multiple control and state buses:} these buses are used to, among other things, monitor the states of the buffers of each computing matrix (to avoid reads of empty buffers or writes of full buffers), parameterize each unit, send the start signal to each matrix , etc.
%\end{itemize}}

\spanish{\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{computation_block.pdf}
	%\centering{
	%	\def\svgwidth{0.4\textwidth}
	%	\input{computation_block.pdf}
	%}
	\caption{Instanciación en paralelo de múltiples unidades de cómputo}
	\label{fig:computation_block}
\end{figure}}

\english{\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{computation_block_eng.pdf}
	%\centering{
	%	\def\svgwidth{0.4\textwidth}
	%	\input{computation_block.pdf}
	%}
	\caption{Parallel instantiation of multiple computation units matrixes}
	\label{fig:computation_block}
\end{figure}}

\spanish{Se destaca un detalle de diseño particular en cuanto a los buffers de cada matriz. Los buffer de datos de imagen, entradas parciales y salidas parciales son buffers de tipo FIFO comunes, pero el buffer de las entradas de coeficientes es un buffer circular. Es decir, se carga con los valores de los coeficientes, y luego en cada lectura el valor leído es re-inyectado a la entrada. Esto se hizo para cargar una vez los valores de los coeficientes necesarios y que se reutilicen automáticamente, sin necesidad de ir a buscarlos a memoria cada vez que son necesarios. Con esto se implementa la reutilización temporal de datos descripta en la sección \ref{section:marcoteorico_aceleradores}.}
\english{A particular design detail is highlighted regarding the buffers of each matrix. Data, partial inputs and partial outputs buffers are common FIFO type buffers, but the buffer for input coefficient is a circular buffer. That is, it is loaded with the values of the coefficients, and then at each reading the read value is re-injected into the input. This was done in order to load the necessary coefficient values only once and have them to be reused automatically, without reading them from memory every time they are needed. This implements the \textit{temporal reuse} of data described in section \ref{section:marcoteorico_aceleradores}.}

\spanish{A su vez, este módulo cuenta con un \textit{generic} que permite sintetizar elementos extras de hardware que verifican dinámicamente si los datos cargados en los buffers de datos o de coeficientes son cero, con el fin de evitar perder ciclos de clock realizando multiplicaciones innecesarias. Esta característica tomó el nombre de \todo{Nombre en proceso}\textit{Dynamic Sparsity Bypass} (de ahora en más, \acronimo).}
\english{In addition, this module can be synthesized with extra hardware elements that dynamically verify if the data loaded in the data or coefficient buffers is zero, in order to avoid losing clock cycles by performing unnecessary multiplications. This feature will be referred during the rest of the paper as \textit{Dynamic Sparsity Bypass} (\acronimo).}

\spanish{\subsubsection{Convolución implementada}}
\english{\subsubsection{Convolution implementation}}

\spanish{El orden en el cual los datos son despachados a este último módulo, y el orden en el cual los resultados de sumas parciales son leídos de el, es decidido por el módulo \textit{traductor de capas} (ver sección \ref{ref:block_diagram}). Los datos de los filtros y los datos a convolucionar son despachados de tal forma que el algoritmo \ref{al:conv} queda implementado tal como explica el pseudocódigo del algoritmo \ref{al:conv_impl}. Este supone que para el cálculo de una determinada capa convolucional se cuenta con la matriz de entrada $i$ con dimensiones $N_{i}\times N_{i}\times N_{if}$, la matriz de coeficientes $k$ con dimensiones $N_{k}\times N_{k} \times N_{if}\times N_{of}]$, el parámetro $stride$ de la capa (el valor $N_{i}$ ya tiene incorporado el $padding$ necesario) y la cantidad de matrices de unidades de cómputo instanciadas en paralelo $N_{cu}$. Esta primera versión del diseño tiene como limitación que solo trabaja con matrices con iguales dimensiones en el eje $x$ e $y$. Es por eso que tanto la matriz $i$, como las matrices $k$ y $output$ tienen las mismas dimensiones en ambos ejes.}
\english{The order in which the data is dispatched to this last module, and the order in which the results of partial sums are read from it, is decided by the \textit{layer translator} module (see section \ref{ref:block_diagram}). The filter data and the data to be convolved are dispatched to the matrix block module with the following limitation: it only works with matrices with equal dimensions on the $x$ and $y$ axis\footnote{Other size aspects should be added in future versions}.}

\spanish{Como se puede ver, el ciclo \textit{for} de la linea \ref{lst:line:for_dsp} representa la paralelización realizada, donde cada matriz de DSPs procesa los mismos datos de entrada pero con filtros distintos. La función DSPSystolicArray representa el procesamiento interno de cada matriz de unidades de cómputo, donde cada una recibe un conjunto de datos de la matriz $i$ de dimensiones $N_{k}\times 4$, junto con el filtro adecuado y un dato que se suma a cada salida. Los ciclos \textit{for} de las líneas \ref{lst:line:for_i} y \ref{lst:line:for_j} representan como se recorre la matriz de entrada $i$ para generar los conjuntos de dimensiones $[N_{k},4]$ que necesita cada matriz.}
\english{Every computation unit matrix receives the same input data but uses different convolution filters. Each one receives a patch of data to process, along with the appropriate filter and data to add to each output.}

%\begin{algorithm*}
%	\tiny
%	\caption{\spanish{Capa convolucional implementada en pseudocódigo}\english{Pseudocode of the convolution implementation on this work}}\label{al:conv_impl}
%	\begin{algorithmic}[1]
%		\Function{ConvImpl}{$i_{[N_{i},N_{i},N_{if}]},k_{[N_{k},N_{k},N_{if},N_{of}]},b_{[N_{of}]},stride,N_{cu}$}
%		
%		\State $output_{[N_{i}/stride,N_{i}/stride,N_{of}]} \leftarrow 0$\Comment{\spanish{Inicialización de la matriz de salida en cero}\english{Output matrix initialization}}
%		
%		\State $temp_{[N_{i}/stride,N_{i}/stride]} \leftarrow 0$\Comment{\spanish{Inicialización de la matriz de salida temporal}\english{Temporal matrix initialization}}
%		
%		\For{$f\gets0$ to $N_{of}-1$ by $N_{cu}$}\Comment{\spanish{Selector de grupo de filtro}\english{Group filter selector}}
%			\For{$k\gets0$ to $N_{if}-1$ by $1$}\Comment{\spanish{Canales de entrada}\english{Loop over the input channels}}
%				\For{$i\gets0$ to $N_{i}-1-N_{k}$ by $stride$} \label{lst:line:for_i} \Comment{\spanish{Eje x de entrada}\english{Loop over the input x axis}}
%					\State $i_{o} \leftarrow i/stride$ \Comment{\spanish{Índice de salida}\english{Output index}}
%					\For{$j\gets0$ to $N_{i}-1-4$ by $2$} \label{lst:line:for_j} \Comment{\spanish{Eje y de entrada}\english{Loop over the input y axis}}
%						\State $j_{o} \leftarrow j/stride$ \Comment{\spanish{Índice de salida}\english{Output index}}
%						
%						\ParFor{$cu\gets0$ to $N_{cu}-1$ by $1$} \label{lst:line:for_dsp} \Comment{\spanish{Procesamiento que realiza cada bloque de matrices}\english{Processing done by each matrix block}}
%							\If{$f = 0$} 
%								\State $temp_{[i_{o},j_{o}]},temp_{[i_{o},j_{o}+1]} \leftarrow$ \Call{DSPSystolicArray}{$i_{[i:i+N_{k}-1,j:j+3,k]},k_{[:,:,k,f+cu]},b_{[f+cu]},b_{[f+cu]}$}
%							\ElsIf{$f = N_{of}-1$}
%								\State $o_{[i_{o},j_{o},f]},o_{[i_{o},j_{o}+1,f]} \leftarrow$ \Call{DSPSystolicArray}{$i_{[i:i+N_{k}-1,j:j+3,k]},k_{[:,:,k,f+cu]},temp_{[i_{o},j_{o}]},temp_{[i_{o},j_{o}+1]}$}
%							\Else
%								\State $temp_{[i_{o},j_{o}]},temp_{[i_{o},j_{o}+1]} \leftarrow$ \Call{DSPSystolicArray}{$i_{[i:i+N_{k}-1,j:j+3,k]},k_{[:,:,k,f+cu]},temp_{[i_{o},j_{o}]},temp_{[i_{o},j_{o}+1]}$}
%							\EndIf
%						\EndParFor
%					\EndFor
%				\EndFor
%			\EndFor
%		\EndFor
%		
%		\State \Return output
%		
%		\EndFunction
%		
%		\Function{DSPSystolicArray}{$i_{[N_{k},4]}$,$k_{[N_{k},N_{k}]}$,$presum_{1}$,$presum_{2}$}
%			\State $out_{1} \leftarrow 0$
%			\State $out_{2} \leftarrow 0$
%			
%			\For{$i\gets0$ to $N_{k}-1$ by $1$}
%				\For{$j\gets0$ to $2$ by $1$}
%					\State $out_{1} \leftarrow out_{1} + i_{[i,j]} \cdot k_{[i,j]}$
%					\State $out_{2} \leftarrow out_{2} + i_{[i,j+1]} \cdot k_{[i,j]}$
%				\EndFor
%			\EndFor
%			
%			\State $out_{1} \leftarrow out_{1} + presum_{1}$
%			\State $out_{2} \leftarrow out_{2} + presum_{2}$
%			
%			\State \Return $[out_{1},out_{2}]$
%			
%		\EndFunction
%	\end{algorithmic}
%\end{algorithm*}

\spanish{Analizando el pseudocódigo presentado, se puede determinar la cantidad mínima teórica de ciclos de clock que puede tardar este diseño en realizar el cálculo completo de una capa convolucional, teniendo en cuenta los parámetros de la capa y la cantidad de bloques de matrices instanciados en paralelo, y a su vez suponiendo que cada bloque siempre tiene datos disponibles para consumir (es decir, nunca entra en un estado \textit{IDLE} ya que siempre tiene datos en sus buffers FIFOs de entrada) y que cada bloque siempre tiene espacio en su buffer de salida para guardar el dato procesado. Siendo $N_{prep}$ la cantidad de ciclos de establecimiento de cada matriz (es decir, cuanto tarda en llenarse el pipeline), $N_{pipeline}$ la cantidad de ciclos de clock que tarda cada matriz en tener datos válidos en su salida (una vez entrada en régimen), $p_x = N_{i}/stride$ la cantidad de grupos de ancho $N_{k}$ que debe procesar cada matriz, $p_y = N_{i}/4$ la cantidad de grupos de 4 datos de alto que debe procesar cada matriz, $ratio = N_{of}/N_{cu}$ la relación entre la cantidad de canales de la matriz de salida y la cantidad de matrices de unidades de cómputo instanciadas, la cantidad mínima de ciclos de clock necesaria para calcular la salida de una capa convolucional se calcula tal como se presenta en la ecuación \ref{eq:ciclos_min}.}
\english{In this work, it is possible to determine the theoretical minimum number of clock cycles that this design may take to perform the complete calculation of a convolutional layer using equation \ref{eq:ciclos_min}, taking into account the parameters of the layer and the number of computation units matrices instantiated in parallel, and also assuming that each matrix always has data available to consume (that is, it never enters an \textit{IDLE} state since it always has data in its input FIFO buffers). It is also supposed that each matrix has \textit{always} space in its output buffer to save the processed data.}

	\spanish{\begin{equation}
		min(ciclos) = N_{prep} + N_{pipeline}\cdot p_x\cdot p_y\cdot N_{if}\cdot ratio
		\label{eq:ciclos_min}
	\end{equation}}
	\english{\begin{equation}
		min(cycles) = N_{prep} + N_{pipeline}\cdot p_x\cdot p_y\cdot N_{if}\cdot ratio
		\label{eq:ciclos_min}
	\end{equation}}
	
\begin{itemize}
	\item $N_{prep}$: the preparation number of cycles of one matrix (this means how many clock cycles it takes to each matrix to fill its internal pipeline with data the first time)
	\item $N_{pipeline}$: the number of cycles that it takes for one matrix to have valid data available at its output
	\item $p_x = N_{i}/stride$: the amount of groups of width equal to $N_{k}$ that each matrix needs to process
	\item $p_y = N_{i}/4$: the amount of groups of height 4 that each matrix needs to process
	\item $ratio = N_{of}/N_{cu}$: the relation between the amount of output channels of the layer and the amount of instantiated computation matrices\footnote{This ratio should be a natural number}
\end{itemize}
%En esta implementación, $N_{est} = 3$ y $N_{pipeline} = 4$. Por lo tanto, la tabla \ref{tab:ciclos_min}

%\begin{table}
%	\centering
%	\scriptsize
%	\begin{tabular}{cccccccc} \toprule
%		$N_{i}$ & $N_{if}$ & $stride$ & $N_{of}$ & $N_{cu}$ & $min(ciclos)$ & t ($f=100MHz$)\\
%		\midrule
%		224 & 3 & 1 & 64 & 12 & \\
%		224 & 64 & 1 & 64 & 12 & \\
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{tab:ciclos_min}
%\end{table}

%Internamente, el chip Z-7010 implementa la arquitectura Zynq, que se presenta en la figura \ref{fig:zynq}. En la parte superior del diagrama se encuentra la sección \textit{Processing System} (en esta sección, de ahora en más llamada PS, se encuentra el ARM Cortex-A9) y en la parte inferior la sección \textit{Programmable Logic} (esta es la sección que contiene la FPGA, de ahora en más llamada PL). A su vez, también se aprecian los puertos de comunicación entre ambas secciones, a los cuales se les dará un tratamiento especial en la sección \ref{section:comunicacion}.

%\begin{figure}
%	\centering
%	\includegraphics[width=0.4\textwidth]{zynq.PNG}
%	\caption{Arquitectura Zynq (para más información, ver \href{https://www.xilinx.com/support/documentation/user_guides/ug585-Zynq-7000-TRM.pdf}{UG585})}
%	\label{fig:zynq}
%\end{figure}

\spanish{\subsection{Diagrama en bloques del proyecto}}
\english{\subsection{Block diagram of the entire architecture}}
\label{ref:block_diagram}

\spanish{\begin{figure}
		\centering
		\includegraphics[width=0.4\textwidth]{bloques_general.pdf}
		\caption{Esquema general del proyecto}
		\label{fig:general}
\end{figure}}

\english{\begin{figure*}[ht]
		\centering
		\includegraphics[width=0.8\textwidth]{bloques_general_eng.pdf}
		\caption{General block diagram of the proposed design}
		\label{fig:general}
\end{figure*}}

\spanish{La figura \ref{fig:general} muestra todos los módulos interconectados entre sí. A continuación se presenta una breve descripción de cada uno de ellos:}
\english{Figure \ref{fig:general} shows all the modules interconnected with each other. A brief description of each of one them is presented:}

	\spanish{\begin{itemize}
		\item \textbf{CPU:} ejecuta un sistema operativo Linux y tiene como tarea obtener la imagen a analizar, avisarle al hardware a través de un driver para que de inicio al procesamiento, y esperar el resultado.
		\item \textbf{CDMA:} este bloque realiza transferencias de datos entre la memoria externa y la memoria interna de la FPGA. 
		\item \textbf{Unidades de cómputo:} este módulo fue descripto en detalle en la sección \ref{section:conv_opt}.
		\item \textbf{Módulos principales:} los módulos controlador, sumador y pooling resuelven cada uno de ellos una capa de una red neuronal convolucional clásica. Obtienen los datos necesarios de la memoria interna, realizan la operación (internamente o enviando los datos al módulo de unidades de cómputo) y guardan nuevamente el resultado en la memoria.
		\item \textbf{Traductor de capas:} este módulo es el que contiene el conocimiento sobre la arquitectura de la red neuronal que se quiere ejecutar (es decir, la sucesión de capas, los tipos de cada capa, los parámetros específicos de cada una, etc), y a su vez se encarga de coordinar el funcionamiento de todos los módulos del desarrollo. Esto permite que el diseño sea configurable, seleccionando la red a ejecutar al momento de implementar el código.
	\end{itemize}}
	\english{\begin{itemize}
		\item \textbf{CPU:} it runs a Linux operating system and its task is to obtain the image to be analyzed, notify the hardware through a driver so that it can start processing, and wait for the result.
		\item \textbf{CDMA:} This block performs data transfers between the external memory and the internal memory of the FPGA.
		\item \textbf{Computation units:} already described in section \ref{section:conv_opt}.
		\item \textbf{Principal modules:} the controller, adder and pooling modules each represent one layer of a classical convolutional neural network. They obtain the necessary data from the internal memory, perform the operation (internally or by sending the data to the matrix block module, section \ref{section:bloque_de_matrices}) and save the result to memory again.
		\item \textbf{Layer translator:} this module is the one that contains the knowledge about the architecture of the neural network to be executed (that is, the layers sequence, the types of each layer, the specific parameters of each one of them, etc.), and it coordinates the operation of all the other modules. This allows the design to be configurable, selecting the network to run when implementing it.
	\end{itemize}}

==> 04-validacion_min.tex <==
\spanish{\section{Validación}}
\english{\section{Validation}}

\spanish{Con el objetivo de validar el funcionamiento del desarrollo de hardware realizado, se entrenó una red neuronal basada en la arquitectura ResNet \cite{resnet1,resnet2} compuesta de 21 capas convolucionales para clasificar imágenes del set de datos CIFAR-10 \cite{cifar10}. Este set de datos contiene 60000 imágenes de 32x32x3 píxeles, dispuestas en 10 categorías mutuamente excluyentes, las cuales se encuentran separadas en 50000 imágenes para entrenar la red y 10000 imágenes para validar el entrenamiento realizado. %La figura \ref{fig:cifar10} muestra algunos ejemplos de las imágenes del set de datos y sus respectivas categorías. Se destaca que el entrenamiento se realiza solamente sobre el conjunto de 50000 imágenes, las restantes 10000 se encuentran separadas y solo se utilizan para obtener la métrica final del entrenamiento de la red.
} 
\english{In order to validate the operation of the developed hardware, a neural network based on the ResNet architecture \cite{resnet1,resnet2} composed of 21 convolutional layers was trained to classify images from the CIFAR-10 dataset \cite{cifar10}. This dataset contains 60,000 images of $32\times32\times3$ pixels, arranged in 10 mutually exclusive categories, which are separated into 50,000 images to train the network and 10,000 images to validate the performed training.}

    %\begin{figure}
    %    \begin{center}
    %        \includegraphics[width=0.4\textwidth]{cifar10.PNG}
    %    \end{center}
    %    \caption[Ejemplos de imágenes del set de datos CIFAR-10]{Ejemplos de imágenes del set de datos CIFAR-10 y sus respectivas categorías}
    %     \label{fig:cifar10}
    %\end{figure}
    
%Para esta implementación se decidió utilizar la arquitectura conocida como ResNet \cite{resnet1,resnet2}.%, la cual esta compuesta de 20 capas convolucionales dispuestas en \textit{cápsulas de residuos} consecutivas \footnote{Para poder implementar esta red utilizando el diseño realizado en hardware, se eliminaron las capas de tipo \textit{Batch Normalization} que si se encuentran presentes en el paper original, ya que la implementación de estas no se encuentran dentro del alcance del proyecto}.

%    \begin{figure*}
%    	\centering
%    	\includegraphics[width=0.6\textwidth]{resnet.pdf}
    	%\centering{
    	%	\def\svgwidth{0.6\textwidth}
    	%	\input{resnet.pdf}}
%    	\caption{Arquitectura ResNet: capas convolucionales (azul), capas de activación de tipo ReLu (verde), capas sumadoras (rosa), capa pooling (amarillo), capa \textit{fully connected} (rojo)}
%    	\label{fig:resnet}
%    \end{figure*}
    
\spanish{\subsection{Entrenamiento}}
\english{\subsection{Training}}

\spanish{En cada versión entrenada se aplicaron las siguientes técnicas:}
\english{In each trained version (see table \ref{tab:resultados_entrenamiento}), the following techniques were used:}

	\spanish{\begin{itemize}
		\item Se aplicó un factor de aprendizaje variable a medida que se avanza en el entrenamiento. Esta técnica se utiliza para converger rápidamente durante las primeras iteraciones del entrenamiento (aplicando un factor de aprendizaje alto que implica modificaciones grandes a los coeficientes de la red), para luego bajar el factor de aprendizaje y aplicar modificaciones más finas a los coeficientes de la red.
		\item A su vez, se utilizó la clase \href{https://keras.io/api/callbacks/reduce_lr_on_plateau/}{ReduceLROnPlateau} \cite{ReduceLROnPlateau} que monitorea constantemente el valor de la función de pérdida y si esta no se reduce luego de una determinada cantidad de épocas (conocidas como \textit{paciencia}), el factor de aprendizaje se reduce por un factor, volviendo luego lentamente a su valor original.
		\item Dado que el set de datos está limitado a 50000 imágenes, se utilizaron técnicas para ampliar el set de datos durante el entrenamiento. Estas técnicas de aumento del set de entrenamiento parten de la premisa que una imagen perteneciente a una determinada clase A sigue perteneciendo a la clase A si por ejemplo: se desplaza cierto porcentaje de píxeles a la izquierda/derecha o arriba/abajo, si se espeja horizontalmente, si se le suma cierto nivel de ruido, etc. Para esto se utilizó la clase \href{https://keras.io/api/preprocessing/image/}{ImageDataGenerator} \cite{ImageDataGenerator} del framework Keras. 
	\end{itemize}}
	\english{\begin{itemize}
			\item A variable learning factor was applied as the training progressed.
			\item The class \href{https://keras.io/api/callbacks/reduce_lr_on_plateau/}{ReduceLROnPlateau} of the Keras framework was used to also dynamically modify the learning factor.
			\item Since the data set is limited to 50,000 images, techniques were used to expand the data set during training. For this, the class \href{https://keras.io/api/preprocessing/image/}{ImageDataGenerator} of the Keras framework was used. 
	\end{itemize}}

%\spanish{El entrenamiento de la red se realizó en 4 etapas claramente diferenciadas, como se presenta en el cuadro \ref{tab:resultados_entrenamiento}: %Se destacan 3 puntos del cuadro: que la técnica de \textit{pruning selectivo} fue desarrollada para esta investigación, que el modelo 2 fue reentrenado a partir del modelo 1, y que los modelos 3 y 4 fueron reentrenados a partir del modelo 2.
%}
%\english{The training of the network was carried out in 4 clearly differentiated stages, as presented in table \ref{tab:resultados_entrenamiento}.}

\begin{table}[H]
	\centering
	\scriptsize
	\begin{tabular}{cccccc} \toprule
		& Framework & \spanish{Representación}\english{Representation} & Pruning & \spanish{Exactitud}\english{Accuracy} [\%] \\
		\midrule
		1 & Keras \cite{Keras} & \spanish{Flotante 32 bits}\english{32 bit floating point} & - & 86,82 \\
		2 & QKeras \cite{QKeras} & \spanish{Punto fijo 8 bits}\english{8 bit fixed point} & - & 86,56 \\
		3 & QKeras \cite{QKeras} & \spanish{Punto fijo 8 bits}\english{8 bit fixed point} & \spanish{Uniforme}\english{Uniform} \cite{zhu2017prune} & 86,65 \\
		4 & QKeras \cite{QKeras} & \spanish{Punto fijo 8 bits}\english{8 bit fixed point} & \textit{HW-aware} & 84,15 \\
		\bottomrule
	\end{tabular}
	\caption{\spanish{Modelos entrenados y métricas resultantes al ejecutar el modelo en la PC}\english{PC training results}}
	\label{tab:resultados_entrenamiento}
\end{table}

	\spanish{\begin{enumerate}
		\item Esta versión fue entrenada desde cero durante 200 épocas (ver figuras \ref{gra:primerversion_entrenamiento}) utilizando la librería de entrenamiento Keras \cite{Keras}, con todos los coeficientes de la red representados en flotantes de 32 bits.
		\item Esta versión fue entrenada a partir de la versión 1 durante 100 épocas (ver figuras \ref{gra:cuantizacion_entrenamiento}), pero con todos los coeficientes representados con valores de punto fijo de 8 bits, utilizando para ello la librería QKeras \cite{QKeras}. Se eligió representar los coeficientes de la red neuronal con 5 bits a la derecha del punto decimal, y con 4 bits para representar las salidas de cada capa.
		\item Esta versión fue entrenada a partir de la versión 2 durante 100 épocas (ver figuras \ref{gra:pruning_entrenamiento}), aplicando la técnica de \textit{pruning} uniforme\cite{zhu2017prune} descripta en la sección \ref{section:marcoteorico_pruning}. Se eligió un porcentaje de pruning del 80\%.
		\item Esta versión fue entrenada a partir de la versión 2 durante 60 épocas (ver figuras \ref{gra:grouped_pruning_entrenamiento}), aplicando una técnica de compresión desarrollada para este proyecto: \textit{hardware-aware pruning}. Los coeficientes a \textit{recortar} se eligen siguiendo el siguiente paradigma: \textit{filtros que se procesan juntos en paralelo, se recortan juntos}\footnote{En inglés va a quedar mejor: \textit{filters that are processed together, are pruned together}}. Dado que las matrices descriptas en la sección \ref{section:bloque_de_matrices} inician su procesamiento al mismo tiempo, y no terminan hasta que la última matriz haya terminado de procesar la cantidad de datos que debe procesar \footnote{Esto será mejorado en futuros proyectos}, se maximiza el efecto de la característica \acronimo si se logra que todos los filtros de un conjunto de filtros que se procesa junto valga cero. Se eligió un porcentaje de pruning del 50\%.
	\end{enumerate}}
	\english{\begin{enumerate}
			\item This version was trained from scratch during 200 epochs (see figures \ref{gra:primerversion_entrenamiento}) using the Keras framework \cite{Keras}, by representing all network weights as floating point values.
			\item This version was trained for 100 epochs using the weights pre-trained in version 1 (see figures \ref{gra:cuantizacion_entrenamiento}), but quantizing them to a 8 bit fixed point representation using the QKeras framework \cite{QKeras}. The decimal point was chosen at 5 (bits to the right of the decimal point) to represent the coefficients of the neural network, and 4 bits for the outputs of each layer.
			\item This version was trained for 100 epochs using the weights pre-trained in version 2 (see figures \ref{gra:pruning_entrenamiento}), by applying the \textit{uniform pruning} technique \cite{zhu2017prune} described in section \ref{section:marcoteorico_pruning}. A target pruning of 80\% was chosen for all layers (this means, 80\% of the weights of each layer were pruned).
			\item This version was also trained using the pre-trained weights of version 2, but it was trained for 60 epochs (see figures \ref{gra:grouped_pruning_entrenamiento}), by applying a pruning technique developed specifically for this project: \textit{hardware-aware pruning}. \todo{Mejorar explicación}The coefficients that are pruned are chosen using the following paradigm: \textit{filters that are processed together, are pruned together}. Since all computation units blocks of the matrix block described in section \ref{section:bloque_de_matrices} start processing at the same time, and they don't finish until the last array has finished processing the amount of data it should process \footnote{This limitation should be improved in future versions} the effect of the \acronimo feature is maximized if all filters in the same filter set are forced to be zero (a filter set is defined as all filters that are processed together in parallel, as it can be seen in the parallel \textit{for} cycle at line \ref{lst:line:for_dsp} of algorithm \ref{al:conv_impl}). A target pruning of 50\% of filter sets was used (this means, 50\% of the filter sets of the entire network were pruned).
	\end{enumerate}}


%Para validar la calidad del entrenamiento se utilizó la métrica conocida como \textit{exactitud}, cuya fórmula de cálculo se puede ver en la ecuación \ref{eq:accuracy}.

%	\begin{equation}
%	Exactitud [\%] = \frac{Cantidad\:de\: predicciones\:correctas}{Cantidad\: total\: de\: predicciones} * 100
%	\label{eq:accuracy}
%	\end{equation}
    
    %\subsection{Resultados del entrenamiento}
    
    %El cuadro \ref{tab:resultados_entrenamiento} muestra los resultados de la exactitud obtenida en la predicción sobre el set de test de CIFAR-10, para los 4 modelos entrenados.
    
    %\begin{table}[H]
    %	\centering
    %	\begin{tabular}{cc} \toprule
    %		Modelo & Exactitud \\
    %		\midrule
    %		1 (original) & 86,82 \\
    %		2 (QKeras) & 86,56 \\
    %		3 (Pruning) & 86,65 \\
    %		4 (Pruning selectivo) & 84,15 \\
    %		\bottomrule
    %	\end{tabular}
    %	\caption{Modelos entrenados y métricas resultantes al ejecutar el modelo en la PC}
    %	\label{tab:resultados_entrenamiento}
    %\end{table}

==> 05-medicion_min.tex <==
\spanish{\section{Medición}}
\english{\section{Measurements}}


{\scriptsize
	\begin{table*}[ht]
		%\todo{revisar!!!!!!!}
		\centering
		\scriptsize
		\begin{tabular}{ccccccccccccc}\toprule
			\multirow{3}{*}{\spanish{Placa}\english{Board}} & \multirow{3}{*}{\spanish{Frecuencia}\english{Frecuency} [MHz]} & \multirow{3}{*}{DSPs} & \spanish{Modelo}\english{Model} & \multicolumn{2}{c}{QKeras (2)} & & \multicolumn{2}{c}{Pruning (3)} & & \multicolumn{3}{c}{\spanish{Pruning selectivo}\english{Hardware-aware pruning} (4)} \\
			
			\cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-13}
			
			& & & \acronimo?  & \spanish{Si}\english{Yes} & No & & \spanish{Si}\english{Yes} & No & & \spanish{Si}\english{Yes} & No & \spanish{Si}\english{Yes} \\
			
			& & & \spanish{Prof. buffer datos}\english{Depth data buffer} & 8 & 8 & & 8 & 8 & & 8 & 8 & 32 \\
			
			\midrule
			
			\multirow{5}{*}{Zybo} & \multirow{5}{*}{70} & \multirow{5}{*}{72} & \spanish{Exactitud}\english{Accuracy} [\%] & 81.88 & 81.88 & & 81.81 & 81.81 & & 79.72 & 79.72 &- \\
			
			& & & \spanish{Diferencia vs PC}\english{Difference vs PC} [\%] & 4.68 & 4.68 & & 4.84 & 4.84 & & 4.43 & 4.43 &- \\
			
			%ROC AUC & \\
			& & & \spanish{Tiempo total}\english{Total time} [s] & 211.70 & 213.39 & & 211.43 & 213.39 & & 193.37 & 213.39 &- \\
			
			& & & \spanish{Tiempo por imagen}\english{Mean time per image} [ms] & 21.17 & 21.34 & & 21.14 & 21.34 & & \textbf{19.34} & 21.34 &- \\
			
			& & & GOPs & 2.173 & 2.156 & & 2.176 & 2.156 & & \textbf{2.379} & 2.156 &- \\
			
			\midrule
			
			\multirow{5}{*}{Zedboard} & \multirow{5}{*}{100} & \multirow{5}{*}{72} & \spanish{Exactitud}\english{Accuracy} [\%] & 81.49 & 81.88 & & 81.63 & 81.81 & & 79.42 & 79.72 & 79.72\\
			
			& & & \spanish{Diferencia vs PC}\english{Difference vs PC} [\%] & 5.07 & 4.68 & & 5.02 & 4.84 & & 4.73 & 4.43 & 4.43 \\
			
			%ROC AUC & \\
			& & & \spanish{Tiempo total}\english{Total time} [s] & 124.93 & 126.33 & & 122.52 & 126.33 & & 70.04 & 126.32 & 64.54 \\
			
			& & & \spanish{Tiempo por imagen}\english{Mean time per image} [ms] & 12.25 & 12.63 & & 12.25 & 12.63 & & 7.00 & 12.63 &\textbf{6,45} \\
			
			& & & GOPs & 3.682 & 3.641 & & 3.754 & 3.641 & & 6.568 & 3.641 &\textbf{7.127} \\
			
			\midrule
			
			\multirow{5}{*}{Zedboard} & \multirow{5}{*}{83.3} & \multirow{5}{*}{144} & \spanish{Exactitud}\english{Accuracy} [\%] & 81.88 & 81.88 & & 81.81 & 81.81 & & 79.72 & 79.72 & 79.72 \\
			
			& & & \spanish{Diferencia vs PC}\english{Difference vs PC} [\%] & 4.68 & 4.68 & & 4.84 & 4.84 & & 4.43 & 4.43 & 4.43 \\
			
			%ROC AUC & \\
			& & & \spanish{Tiempo total}\english{Total time} [s] & 107.10 & 107.81 & & 106.19 & 107.83 & & 66.70 & 107.81 & 61.60 \\
			
			& & & \spanish{Tiempo por imagen}\english{Mean time per image} [ms] & 10.71 & 10.78 & & 10.62 & 10.78 & & 6.67 & 10.78 & \textbf{6.16} \\
			
			& & & GOPs & 4.295 & 4.227 & & 4.332 & 4.266 & & 6.897 & 4.267 & \textbf{7.468} \\
			
			\bottomrule
			
		\end{tabular}
		\caption{\spanish{Resultados de distintas versiones del diseño ejecutados sobre 2 FPGAs distintas}\english{Results of different versions of the design executed on 2 different FPGA development boards}}
		\label{tab:resultados}
\end{table*}}

\spanish{Para la ejecución de la red entrenada sobre el hardware diseñado, se implementaron múltiples versiones (los reportes de uso de recursos de cada versión se encuentran en las figuras \ref{fig:implementacion} y \ref{fig:implementacion2}), cada una de ellas parametrizada de forma distinta y con la RAM interna de la FPGA precargada con los coeficientes de uno de los 3 modelos cuantizados presentados en la sección anterior.}
\english{For the execution of the trained networks on the designed hardware, multiple versions were implemented (for the resource usage reports of each version see figures \ref{fig:implementacion} and \ref{fig:implementacion2}), each one of them parameterized in a different way and with the internal RAM of the FPGA preloaded with the coefficients of one of the 3 quantized models presented in the previous section.}

\pgfplotstableread[row sep=\\, col sep=&]{
	resource & Zybo12-DSPSI & Zybo12-DSPNO & Zedboard12-DSPNO & Zedboard12-DSPSI & Zedboard24-DSPNO & Zedboard24-DSPSI \\
	LUT & 89.32 & 90.52 & 39.28 & 39.07 & 63.95 & 63.01\\
	%LUTRAM & 13.82 & 13.82\\
	FF & 31.36 & 31.38 & 12.68 & 12.05 & 17.92 & 17.92\\
	BRAM & 94.2 & 94.2 & 52.1 & 52.1 & 54.6 & 54.6\\
	DSP & 90 & 90 & 32.73  & 32.73 & 65.45 & 65.45\\
}\ResourceData
\begin{figure}
	\centering
	\begin{tabular}{cc}
		\subfloat[]{
			\begin{tikzpicture}[scale=0.5]
			\begin{axis}[ybar,
			bar width=.25cm,
			title={\spanish{Reporte de implementación Zybo}\english{Zybo implementation report}},
			width=0.4\textwidth,
			height=0.4\textwidth,
			legend style={at={(0.35,0.95)}, anchor=north, legend columns=1},
			symbolic x coords={LUT,FF,BRAM,DSP},
			xtick=data,
			enlarge x limits={abs=0.5cm},
			nodes near coords,
			nodes near coords style={rotate=90, anchor=west},
			nodes near coords align={vertical},
			ylabel near ticks,
			ymin=0,ymax=120,
			ylabel={\spanish{Porcentaje}\english{Percentage} [\%]},
			ymajorgrids=true,
			]
			\addplot table[x=resource, y=Zybo12-DSPSI]{\ResourceData};
			\addplot table[x=resource, y=Zybo12-DSPNO]{\ResourceData};
			\legend{\acronimo? No, \acronimo? \spanish{Si}\english{Yes}}
			\end{axis}
			\end{tikzpicture}
		} &
		\subfloat[]{
			\begin{tikzpicture}[scale=0.5]
			\begin{axis}[ybar,
			bar width=.25cm,
			title={\spanish{Reporte de implementación Zedboard}\english{Zedboard implementation report}},
			width=0.5\textwidth,
			height=0.4\textwidth,
			legend style={at={(0.69,0.95)}, anchor=north, legend columns=2},
			symbolic x coords={LUT,FF,BRAM,DSP},
			xtick=data,
			enlarge x limits={abs=0.8cm},
			nodes near coords,
			nodes near coords style={rotate=90, anchor=west},
			nodes near coords align={vertical},
			ylabel near ticks,
			ymin=0,ymax=120,
			ylabel={\spanish{Porcentaje}\english{Percentage} [\%]},
			ymajorgrids=true,
			]
			\addplot table[x=resource, y=Zedboard12-DSPSI]{\ResourceData};
			\addplot table[x=resource, y=Zedboard12-DSPNO]{\ResourceData};
			\addplot table[x=resource, y=Zedboard24-DSPSI]{\ResourceData};
			\addplot table[x=resource, y=Zedboard24-DSPNO]{\ResourceData};
			\legend{\acronimo? No, \acronimo? \spanish{Si}\english{Yes},\acronimo? No, \acronimo? \spanish{Si}\english{Yes}}
			\end{axis}
			\end{tikzpicture}
		} 
	\end{tabular}
	\caption{\spanish{Uso de recursos para las distintas versiones del diseño implementadas para una profundidad del buffer de entrada de 8, parametrizadas por el parámetro \acronimo}\english{Resource usage for the different versions of the design implemented for an input data buffer depth of 8 elements, parameterized by the \acronimo parameter}}
	\label{fig:implementacion}
\end{figure}

\pgfplotstableread[row sep=\\, col sep=&]{
	resource & Zedboard12-8 & Zedboard12-32 & Zedboard24-8 & Zedboard24-32 \\
	LUT & 39.07 & 39.87 & 63.95 & 64.84\\
	%LUTRAM & 13.82 & 13.82\\
	FF & 12.05 & 12.27 & 17.92 & 18.37\\
	BRAM & 52.1 & 52.1 & 54.6 & 54.6\\
	DSP & 32.73  & 32.73 & 65.45 & 65.45\\
}\ResourceDataBis
\begin{figure}
	\centering
	\begin{tabular}{c}
		\subfloat[]{
			\begin{tikzpicture}[scale=0.5]
			\begin{axis}[ybar,
			bar width=.25cm,
			title={\spanish{Reporte de implementación Zedboard}\english{Zedboard implementation report}},
			width=0.6\textwidth,
			height=0.4\textwidth,
			legend style={at={(0.72,0.95)}, anchor=north, legend columns=2},
			symbolic x coords={LUT,FF,BRAM,DSP},
			xtick=data,
			enlarge x limits={abs=0.8cm},
			nodes near coords,
			nodes near coords style={rotate=90, anchor=west},
			nodes near coords align={vertical},
			ylabel near ticks,
			ymin=0,ymax=120,
			ylabel={\spanish{Porcentaje}\english{Percentage} [\%]},
			ymajorgrids=true,
			]
			\addplot table[x=resource, y=Zedboard12-8]{\ResourceDataBis};
			\addplot table[x=resource, y=Zedboard12-32]{\ResourceDataBis};
			\addplot table[x=resource, y=Zedboard24-8]{\ResourceDataBis};
			\addplot table[x=resource, y=Zedboard24-32]{\ResourceDataBis};
			\legend{Zybo: 8,Zybo: 32,Zedboard: 8,Zedboard: 32}
			\end{axis}
			\end{tikzpicture}
		}
	\end{tabular}
	\caption{\spanish{Uso de recursos para las distintas versiones del diseño implementadas con el parámetro \acronimo activado, parametrizadas por la profundidad del buffer de datos de cada matriz de DSPs}\english{Resource usage for the different versions of the design implemented with the \acronimo parameter activated, parameterized by the depth of the data buffer of each array of DSPs}}
	\label{fig:implementacion2}
\end{figure}

%\begin{enumerate}
%	\item Versión con la RAM interna de la FPGA precargada con los coeficientes cuantizados del modelo 2.
%	\item Versión con la RAM interna de la FPGA precargada con los coeficientes cuantizados y aplicando la técnica de pruning uniforme del modelo 3.
%	\item Versión con la RAM interna de la FPGA precargada con los coeficientes cuantizados y aplicando la técnica de pruning selectivo del modelo 4.
%\end{enumerate}

%Los modelos sintetizados e implementados se configuraron para trabajar a 70 MHz. Si se sigue subiendo la frecuencia de trabajo, comienzan a aparecer errores de \textit{timing} ya que se están utilizando casi el 100 \% de los recursos de la FPGA. El estudio de los errores de \textit{timing} y las posibles mejoras que permitan subir la frecuencia de operación serán investigadas en futuras versiones del proyecto.

\spanish{A modo de comparación, se procesaron las 10000 imágenes del set de test de CIFAR-10 sobre la FPGA para las distintas versiones implementadas, obteniéndose los resultados presentados en el cuadro \ref{tab:resultados}. La fila \textit{Prof. buffer datos} indica el tamaño de uno de los buffers FIFO que comunican el módulo principal \textit{Controlador} con el módulo de \textit{unidades de cómputo}. La fila \textit{GOPs} muestra la cantidad de giga-operaciones por segundo que alcanza a realizar cada versión, que se calcula como la cantidad total de operaciones que debe realizar la red neuronal elegida (para la red ResNet20 elegida y para el set de datos elegido, son 0,046 GOP) sobre el tiempo promedio que se tarda en procesar una imagen.}
\english{The 10,000 images of the CIFAR-10 test set were processed on the FPGA for the different implemented versions, obtaining the results presented in table \ref{tab:resultados}. The \textit{Depth data buffer} row indicates the size of the FIFO buffers that communicate the \textit{Controller} module with the \textit{computation units}. %The \textit{GOPs} row indicates the amount of giga-operations per second that each version is able to achieve, which is calculated as the total amount of operation that the selected neural network needs to do to process one image (for this network and the selected datasets image size, this are 0,046 GOP) divided by the mean time that it takes for the hardware to process one image.
}

\spanish{Finalmente, se compara el desarrollo realizado con otros aceleradores de hardware. El cuadro \ref{tab:comparison} presenta distintos desarrollos de implementaciones de redes neuronales convolucionales sobre FPGAs. Cabe destacar que aunque parece haber grandes diferencias entre este proyecto y otros desarrollos, los otros proyectos no solamente trabajan a frecuencias mayores, sino que también utilizan muchos mas DSPs, y también FPGAs con mayor cantidad de recursos.}
\english{Finally, in table \ref{tab:comparison} this project is compared against other hardware accelerators. It should be noted that although there seem to be great differences between this project and other developments, the other projects not only work at higher frequencies, but also use many more DSPs and FPGAs with a greater amount of resources.}

\begin{table}[H]
	\centering
	\scriptsize
	\begin{tabular}{ccccc}\toprule
		\spanish{Desarrollo}\english{Work} & Chip & \spanish{Frecuencia}\english{Frequency} [MHz] & DSPs & GOPs\\
		\midrule
		\spanish{Este desarrollo}\english{This work} & XC7Z010 & 70 & 72 & 2.397 \\
		\spanish{Este desarrollo}\english{This work} & XC7Z020 & 100 & 72 & 7.127 \\
		\spanish{Este desarrollo}\english{This work} & XC7Z020 & 83.3 & 144 & 7.468 \\
		\cite{7930521} & XC7Z020 & 214 & 190 & 84.3 \\
		\cite{7930521} & XC7Z030 & 150 & 400 & 105.2 \\
		\cite{10.1145/2847263.2847276} & 5SGSD8 & 120 & 1963 & 117.8 \\
		\cite{7929190} & VX690T & 100 & 1436 & 222.1 \\ 
		\bottomrule
	\end{tabular}
	\caption{\spanish{Comparación de distintos diseños de aceleradores de hardware que trabajan en 8 bits}\english{Comparison of different 8-bit hardware accelerators designs}}
	\label{tab:comparison}
\end{table}

==> 06-conclusiones_min.tex <==
\spanish{\section{Conclusiones}}
\english{\section{Conclusions}}

%\spanish{Partiendo del cuadro \ref{tab:resultados} se puede extraer un conjunto de conclusiones que permiten analizar el desarrollo realizado, las cuales serán presentadas en esta sección.}
%\english{By analyzing table \ref{tab:resultados}, a set of conclusions will be presented in this section, which allow us to characterize this development, and explain its advantages, disadvantages, and future work.}

\spanish{Por un lado, se aprecia que para el modelo \textit{QKeras} (modelo 2), el hecho de activar o no activar la función \acronimo \textbf{no aporta una mejora significativa} en el tiempo de inferencia por imagen del diseño (la diferencia es de solamente el 0.79 \%). Esto es esperable, ya que este modelo no fue entrenado con ninguna técnica de \textit{pruning}, y por lo tanto los coeficientes de sus filtros no tienen ninguna restricción aplicada para forzarlos a cero y de esta forma poder aprovechar la característica \acronimo.}
\english{On one hand, for the \textit{QKeras} model (2), the activating of the \acronimo feature \textbf{does not add a significant improvement} to the mean inference time per image (this difference is as small as 0.79\%). This was expected and not at all surprising, since this model was not trained with any \textit{pruning} technique, and therefore the coefficients of its filters do not have any restriction applied to force them to zero and thus be able to take advantage of the \acronimo feature of the hardware.}

\spanish{También se aprecia que el modelo entrenado con la técnica de \textit{pruning} uniforme \cite{zhu2017prune} (modelo 3) tiene una \textbf{ligera mejora} respecto del anterior entre las versiones con y sin \acronimo (la diferencia es del 3 \% en el mejor de los casos). Sin embargo, esta diferencia \textbf{sigue siendo muy pequeña}.%, sobre todo teniendo en cuenta que este modelo fue entrenado con un factor de pruning objetivo de \textbf{80\%} (es decir, el 80\% de los coeficientes totales de la red valen cero). %¿A que se debe que esta diferencia no sea mayor? Se debe a que este método de pruning uniforme no tiene en cuenta que coeficientes deben ser recortados para maximizar el efecto de esta característica del hardware.
}
\english{It is also appreciated that the model trained with the uniform \textit{pruning} technique (model 3) adds a \textbf{slight improvement} when compared to the previous model, if versions with and without the \acronimo feature are compared (the difference is around a 3\% in the best case). However, this difference \textbf{is still very small}.}

\spanish{Para el modelo entrenado con la técnica de \textit{hardware-aware pruning} (modelo 4), se aprecia una \textbf{notable disminución} del tiempo de inferencia por imagen del diseño que ronda el \textbf{45\%} en el mejor caso cuando se activa el \acronimo. Es de destacar que este modelo había sido entrenado con un pruning objetivo de solamente \textbf{50\%}, y sin embargo \textbf{obtiene mejores resultados} que el modelo 3 en cuanto a velocidad de inferencia, a costa de una mínima pérdida de exactitud.% (el cual no tiene aplicado ninguna técnica de pruning). Es de destacar que este modelo había sido entrenado con un pruning objetivo de solamente \textbf{50\%}, y sin embargo \textbf{obtiene mejores resultados} que el modelo 3 en cuanto a velocidad de inferencia, a costa de una mayor pérdida de exactitud.
}
\english{For the model trained with the \textit{hardware-aware pruning} technique (model 4), a \textbf{notable decrease} in the mean inference time per image of the design is observed, which is around \textbf{45 \%} in the best case, when feature \acronimo is activated. It is noteworthy that this model had been trained with a target pruning of only \textbf{50 \%}, and yet \textbf{obtained better results} than model 3 in terms of inference speed, at the cost of a slight loss of accuracy.}

\spanish{Para el modelo 4 se comparó el tiempo de inferencia por imagen para una profundidad del buffer FIFO de datos de cada unidad de cómputo de 8 y de 32. Si este buffer es muy pequeño, se ocasionan \textbf{tiempos muertos} en las máquinas de estado internas del módulo \textit{Controlador} que aumentan el tiempo de inferencia total por imagen. Tal como se pone de manifiesto en la tabla, un diseño implementado con sus buffers de datos de 32 elementos de profundidad logra una mejora del 8\%. Pero por otro lado, este aumento de la profundidad trae aparejado un aumento del uso de recursos de la FPGA (figura \ref{fig:implementacion2}). Por lo tanto, pese a que en este caso la mejora es \textbf{pequeña}, si se cuenta con una \textbf{FPGA con mayores recursos} se puede conseguir una mejora considerable aumentando aún más el tamaño de este buffer.}
\english{For model 4, the inference time per image was compared for a FIFO data buffer depth (for each computation unit) of 8 and 32 elements. If this buffer is too small, \textbf{idle times} appear in the internal state machines of the \textit{Controller} module, thus increasing the mean inference time per image. As shown in the table, a design implemented with 32-element deep data buffers achieves an 8 \% improvement in the inference speed. But on the other hand, this depth increase also brings with it an increase in the FPGA resource usage (figure \ref{fig:implementacion2}). Therefore, although the improvement is \textbf{small} in this particular case, if there are \textbf{FPGA with more resources} available, a considerable improvement can be obtained by increasing the size of this buffer even more.}

%También se puede determinar un \textit{factor de paralelización} ($f_{p}$), que indica en que medida paraleliza las operaciones matemáticas este diseño a comparación de un diseño completamente secuencial ideal (que pueda realizar una operación matemática por ciclo de clock). Este factor $f_{p}$ se puede calcular como el tiempo que tarda este sistema secuencial en procesar una imagen (es decir, las 0,046 GOP) dividido el tiempo que tarda este diseño de hardware sobre FPGA en hacerlo. El resultado da $f_{p} \approx 34$, lo cual pone de manifiesto los frutos de las decisiones tomadas durante el proyecto en cuanto a la paralelización de operaciones matemáticas.

\spanish{\section{Futuros trabajos}}
\english{\section{Future work}}

\spanish{Este trabajo abre las puertas a un gran conjunto de futuras investigaciones, donde se analizarán extensiones y mejoras a este desarrollo. Por un lado, se investigará el uso de los DSP slices en modo SIMD, y en cuanto mejora esto la paralelización del diseño. Por otro lado, el análisis de consumo de energía de estas implementaciones y su relación con el \textit{hardware-aware pruning} y el \acronimo también son temas pendientes que vale la pena investigar. Además, es de interés analizar en detalle a que se debe la poca mejora en el tiempo de procesamiento por imagen para una red entrenada con la técnica estándar de \textit{pruning}, y revisar si se puede mejorar la característica \acronimo para redes entrenadas con esta técnica. Por otro lado, en esta versión del diseño, los coeficientes de la red neuronal a ejecutar se encuentran guardados en la memoria interna sin ningún tipo de compresión, lo cual no es eficiente en redes \textit{pruneadas}. El análisis de técnicas dinámicas de compresión y decompresión de estos datos y su integración en esta arquitectura también son de interés. Finalmente, en futuros trabajos se demostrará la flexibilidad de este diseño, ejecutando múltiples arquitecturas de redes neuronales.}
\english{This work opens the doors to a large set of future research branches, where extensions and improvements to this hardware accelerator will be analyzed. On the one hand, the use of the DSP slices in SIMD mode will be investigated, and how much this improves the parallelization features of the design. On the other hand, the energy consumption analysis of these implementations and its relationship with the \textit{hardware-aware pruning} and the \acronimo feature are also pending topics worth investigating. In addition, it is of great interest to analyze with more detail why a network trained with the standard \textit{pruning} technique has so little improvement in the image processing time, and to review if the \acronimo characteristic can be improved for networks trained with this technique. On the other hand, in this version of the design, the coefficients of the neural network are stored in the internal memory without any type of compression, which is not efficient when executing \textit{pruned} networks. The analysis of dynamic compression and decompression techniques for these data and their integration into this architecture are also of interest. Finally, future work will demonstrate the flexibility of this design, running multiple different neural network architectures.}

%Se concluye por lo tanto que luego de la investigación y el desarrollo realizados, se logró implementar un acelerador de hardware para redes neuronales convolucionales \textbf{completamente funcional}, capaz de ejecutar redes neuronales de una variedad de arquitecturas distintas. Además se verificó que la técnica de \textit{pruning} uniforme \textbf{no} acelera la ejecución de la predicción en el hardware. Para lograr esto, hubo que encontrar \textbf{otra} técnica de \textit{pruning} que aportó cierta pérdida de exactitud en la predicción, pero \textbf{maximizó} el efecto de la característica del hardware de \textit{no} activar los DSPs cuando las entradas de coeficientes son cero. %Finalmente, se concluye que la diferencia que se puede apreciar entre la exactitud de los modelos ejecutados sobre la FPGA contra el mismo modelo ejecutado en la PC utilizando la librería \textit{QKeras} son a causa del framework de entrenamiento que, dado que esta construido sobre otro framework que realiza cálculos utilizando toda la precisión disponible en la PC, es incapaz de simular internamente la aritmética elegida para el proyecto.

==> Makefile <==
export LC_ALL=C

TEX=paper_min_v3.tex  paper_body_v3.tex #Agregar eventualmente algun otro tex
PDF=paper_min_v3

### Don't touch beyond this point.

PDF_N=$(PDF).pdf
# PDF_H=$(PDF)-handout.pdf
#OUTPUT=$(PDF_N) $(PDF_H)

# LaTeX flags
TEXFLAGS=-file-line-error -interaction=nonstopmode

book: $(PDF_N)

#all: $(PDF_N) $(PDF_H)

#handout: $(PDF_H)

$(PDF_N): $(TEX) Makefile
	cd img; make
	-pdflatex $(TEXFLAGS) -jobname $(PDF) $<
	-bibtex $(PDF).aux
	-pdflatex $(TEXFLAGS) -jobname $(PDF) $<
	-pdflatex $(TEXFLAGS) -jobname $(PDF) $<

#$(PDF_H): $(TEX)
#	echo '\PassOptionsToClass{handout}{beamer}\input{$<}' | pdflatex $(TEXFLAGS) -jobname $(PDF)-handout 

clean:
	#rm -f *.aux *.log *.out *.toc *.nav *.snm $(PDF).pdf $(PDF)-handout.pdf
	rm -f *.bbl *.blg *.aux *.log *.out *.toc *.nav *.snm *.pdf *-handout.pdf

